Computability in the Lattice of Equivalence Relations

We investigate computability in the lattice of equivalence relations on the natural numbers. We mostly investigate whether the subsets of appropriately defined subrecursive equivalence relations -for example the set of all polynomial-time decidable equivalence relations- form sublattices of the lattice.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{G. Bonfante, G. Moser (Eds.): 8th Workshop on Developments in\\ Implicit Computational complExity and 5th Workshop on Foundational\\ and Practical Aspects of Resource Analysis
(DICE-FOPARA 2017)\\
EPTCS 248, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.248.8}{10.4204/EPTCS.248.8}}

